Natural SQL: Making SQL Easier to Infer from Natural Language Specifications

Addressing the mismatch between natural language descriptions and the corresponding SQL queries is a key challenge for text-to-SQL translation. To bridge this gap, we propose an SQL intermediate representation (IR) called Natural SQL (NatSQL). Specifically, NatSQL preserves the core functionalities of SQL, while it simplifies the queries as follows: (1) dispensing with operators and keywords such as GROUP BY, HAVING, FROM, JOIN ON, which are usually hard to find counterparts for in the text descriptions; (2) removing the need for nested subqueries and set operators; and (3) making schema linking easier by reducing the required number of schema items. On Spider, a challenging text-to-SQL benchmark that contains complex and nested SQL queries, we demonstrate that NatSQL outperforms other IRs, and significantly improves the performance of several previous SOTA models. Furthermore, for existing models that do not support executable SQL generation, NatSQL easily enables them to generate executable SQL queries, and achieves the new state-of-the-art execution accuracy.

==> qu.tex <==
\section{Question Unifying}
% \subsection{Question Unifying}
% Although IR has been widely used for complex SQL, enthusiasts of end-to-end model expect the text-to-SQL model to automatically distinguish whether the word token `\emph{or}' in Figure \ref{iue-gap} corresponds to \textit{UNION} or \textit{OR} keyword. 
\begin{table}[t]
    \centering
   
    \resizebox{.99\columnwidth}{!}{
    \smallskip\begin{tabular}{cl}
      Question:& How many concerts in 2014 or after? \\\hline
  
   Gold SQL: & {\bf SELECT} count(*) {\bf FROM} concerts 
   \\ & {\bf WHERE} year >= 2014
    \\\hline
  
   Wrong   &  {\bf SELECT} count(*) {\bf FROM} concerts \\ Prediction: &  {\bf WHERE} year > 2014  \\\hline

    \end{tabular}
    }
    \caption{A \textit{WHERE} condition that can easily be predicted incorrectly.}
    \label{table:prediction-error}
\end{table}

Table \ref{table:prediction-error} presents an example that is incorrectly predicted by many models. 
The reason for this prediction error is that the word~`\emph{after}' in most training samples correspond to the `$>$' operator, and the word~`\emph{or}' is mostly used to connect two conditions.
Such a prediction error, as well as examples in Figure \ref{iue-gap}, illustrate the insufficient ability in language understanding and reasoning.

% The schema linking process discussed above is designed for capturing the information about schema items in the natural language question. Meanwhile, conditions are also important for an SQL query. Therefore, we design the question unifying step to improve the condition generation.

We unify the descriptive phrases of three comparative operators, i.e., `\emph{>=}', `\emph{<=}', and `\emph{like}'.
We design several regular expressions to locate all these phrases, and then replace their original descriptive phrases with three unified vague phrases separately. For example, let `[GE]' be the placeholder token representing the `\emph{>=}' operator, then the question in Table \ref{table:prediction-error} can be unified as `\emph{How many concerts [GE] 2014?}'. Similarly, another question `\emph{Which countries have at least 3 cities?}' is unified as `\emph{Which countries [GE] 3 cities?}'.
%  ~\xinyun{TODO: explain what ``shinier'' means, it is just a placeholder token.}

% Due to the limited types of SQL condition operators, the common description about SQL condition is much narrower than other NL tasks. We choose three 

% We unify the question representation corresponding to `$>=$', `$<=$', and `like' SQL operators based on regular expression, because the predictions of neural models tend to be more problematic for these three operators. 
% For example, the sub-question `whose age is or above 20' in Figure \ref{figure1} corresponds to `age $>=$ 20'. The main difficulty comes from the fact that this sub-question includes the word `or', which could also be used to connect parallel conditions. To modify `is or above' to a uniform representation without the word `or', we use the pattern `* or GR' to match `in or above', and this pattern also applies to other phrases such as `equal or bigger'. The unified target representation should use the words that are not easily confused with other expressions, or even create a new word.

% \subsection{Question Repair}
% Since we generate `COL', `TABLE' and `DB' pattern tokens based on the exact match, when the question includes typos for schema-related words, it may cause errors for schema linking. To tackle this issue, before the schema linking process, we first perform a question repair step. Specifically, for each question word token, we retrieve it from a vocabulary of the 20,000 most common English words~\footnote{We download the vocabulary from~\url{https://github.com/first20hours/google-10000-english}.}. If a word is not included in the vocabulary, and its Levenshtein distance~\cite{editdistance} from a database or schema word is equal to 1, we correct the question word accordingly.
